Quadratic Optimization-Based Nonlinear Control for Protein Conformation Prediction

Predicting the final folded structure of protein molecules and simulating their folding pathways is of crucial importance for designing viral drugs and studying diseases such as Alzheimer's at the molecular level. To this end, this paper investigates the problem of protein conformation prediction under the constraint of avoiding high-entropy-loss routes during folding. Using the well-established kinetostatic compliance (KCM)-based nonlinear dynamics of a protein molecule, this paper formulates the protein conformation prediction as a pointwise optimal control synthesis problem cast as a quadratic program (QP). It is shown that the KCM torques in the protein folding literature can be utilized for defining a reference vector field for the QP-based control generation problem. The resulting kinetostatic control torque inputs will be close to the KCM-based reference vector field and guaranteed to be constrained by a predetermined bound; hence, high-entropy-loss routes during folding are avoided while the energy of the molecule is decreased.

==> section/CLFQP.tex <==
\section{CLF-based Quadratic Program Solution}

\begin{itemize}
	\item This is the trivial solution after the zero dynamics analysis 
	is done. However, it lacks a proper geometric insight. Indeed, this control 
	strategy makes the robot to converge to the zero dynamics manifold in a direction perpendicular 
	to the manifold.  
\end{itemize}

==> section/ContProbFormulation.tex <==
\section{Control Problem Formulation and Solution Strategy}
\label{sec:ContProb}

In this section we formulate the straight-line 
path following control problem for swimming magnetic
helical microrobots and outline our solution 
strategy. 

\textbf{Straight-Line Path Following Control (LFC) Problem.} Consider a 
planar magnetic microswimmer whose dynamics are given by~\eqref{eq:2D_dynb}. 
Given a step-out frequency $f_{\text{SO}}$ and direction vector 
%
\[
\hat{e}_{_{\theta_\tx{r}}} = \begin{bmatrix}  \cos(\theta_\tx{r}) \\ \sin(\theta_\tx{r}) \end{bmatrix},
\] 
%
for some constant angle $\theta_r$, make the microrobot to 
converge to the line 
\begin{equation}\label{eq:line}
\mathcal{P}:=\{ p \in \mathbb{R}^2 : p = \tau\hat{e}_{_{\theta_\tx{r}}} ,\, \tau\in \mathbb{R} \}, 
\end{equation}
and to traverse it with a bounded velocity such 
that $|u(t)|\leq f_{\text{SO}}$ for all $t\geq 0$.

Given the path $\mathcal{P}$ in~\eqref{eq:line}, we consider the output 
%
\begin{equation}\label{eq:output}
y = h(p) := \hat{e}_{_{\theta_\tx{r}}}^{\perp^\top} p,
\end{equation}
%
\noindent for the dynamical system in~\eqref{eq:2D_dynb}, where 
%
\[
\hat{e}_{_{\theta_\tx{r}}}^{\perp} =  \begin{bmatrix} -\sin(\theta_\tx{r}) \\  \cos(\theta_\tx{r}) \end{bmatrix},
\]
is the unit vector perpendicular to path $\mathcal{P}$. Indeed, the 
zero level set of the output in~\eqref{eq:output} is the path 
$\mathcal{P}$ in~\eqref{eq:line}.  
%

\noindent\textbf{Solution Strategy.}  Our solution to microrobot LFC 
problem unfolds in the following steps.
%
\begin{itemize}
	\item[] \textbf{Step 1:} In Section~\ref{subsec:zerodyn}, we find the necessary and sufficient 
	condition by which the path $\mathcal{P}$ in~\eqref{eq:line} can 
	be made invariant via the choice of a proper control input for the microrobot closed-loop 
	dynamics. This invariance property ensures that once the 
	microrobot is initialized on $\mathcal{P}$, it will remain on it 
	for all future time. Furthermore, we derive the constrained dynamics of the microswimmer on
    path $\mathcal{P}$.
	
	\item[]  \textbf{Step 2:} In Section~\ref{subsec:los}, we consider the reference model  
	\begin{equation}
	\label{eq:refmodel}
	\dot{p} = \alpha_{\tx{d}}v^{\tx{d}}(p), 
	\end{equation}
	where $\alpha_{\tx{d}}$ is a positive constant and $v^{\tx{d}}(p)$ is the desired closed-loop 
	vector field coming from a line-of-sight guidance law. The constant 
	parameter in guidance law~\eqref{eq:refmodel} is determined by the 
	constrained dynamics of the microrobot on $\mathcal{P}$ obtained in 
	Step 1. We prove that LFC problem objective is achieved for the reference 
	model in~\eqref{eq:refmodel}. 
	%
	\item[] \textbf{Step 3:}  Having obtained a desired closed loop vector field 
	that achieves the LFC objective in Step~2, we cast the control problem as an ODS-based 
	quadratic program in Section~\ref{subsec:ods}. This ODS-based quadratic program 
	minimizes,  at each point $p$ of the state space, the difference between the open-loop and the reference 
	model vector fields in~\eqref{eq:2D_dynb} and~\eqref{eq:refmodel}, while 
	respecting the control input constraints. 
	%
	% perform a zero dynamics analysis for the 
	%output in~\eqref{eq:output}. In particular, we provide necessary and sufficient 
	%conditions for the output to have well-defined relative degree and 
	%derive the induced zero dynamics.	
	%	
\end{itemize}


%\begin{itemize}
%	\item[L1] \textbf{Step-out frequency:}   In particular, we have the 
%	constraint 
%	\begin{equation}
%	\label{eq:stepout}
%	|u| \leq f_{\text{SO}}, 
%	\end{equation}
%	on the control input, where $f_{\text{SO}}$ is the step-out frequency. The step-out 
%	frequency for each microswimmer is known \emph{a priori}. 
%	%
%	%	\item[L2] \textbf{Underactuation:} As it can be seen from the 
%	%	microswimmer's dynamics in~\eqref{eq:2D_dynb}, we have the two degrees of freedom
%	%	$p_x$ and $p_z$, and only one control input. Therefore, the degree of underactuation of 
%	%	the control system given by~\eqref{eq:2D_dynb} is equal to one. 
%	%
%	\item[L2] \textbf{Non-neutrally buoyant bodies:} This problem, which becomes more 
%	significant in  the context of 3D microrobot control, is due to limitations of the optical 
%	microscopes used for sensing the position and orientation of the microrobot. In this document, however, 
%	we assume that the orientation of the microrobot in the $x-z$ plane is known. 
%\end{itemize}
%
%(Alireza: Talk about other papers achievements and drawbacks in control.) 

==> section/conclusion.tex <==
\section{Concluding Remarks and Future Research Directions}
\label{sec:conc}

Using an ODS-based approach, we presented an optimization-based control solution for 
path following control of swimming helical magnetic 
microrobots subject to control input constraints. An LOS-based 
reference model was chosen for the ODS-based quadratic program. 
The proposed control methodology leads us to further research avenues 
for controlling helical magnetic microrobots such as way-point tracking 
control in the cluttered areas of the human body,  three-dimensional 
maneuvering control, control in the presence of disturbances such as 
vessel blood flow, and control of a collection of microrobots moving 
in a formation. 

==> section/dynmodel.tex <==
\section{Dynamical Model}
\label{sec:dynmodel} 
%
Figure~\ref{fig:micro} depicts the configuration of a 
generic helical microrobot. The robot geometry is completely determined by the number of turns of 
the helix $n_\tx{h}$, the helix pitch angle $\theta_\tx{h}$, the helix radius $r_\tx{h}$, and the 
magnetic head radius $r_\tx{m}$.  The helix coordinate frame $x_\tx{h} - z_\tx{h}$ is   
attached to the helix center $O_\tx{h}$.  We also fix a right-handed inertial coordinate frame
in the Euclidean space and denote it by $W$.  We denote the unit vectors in the 
direction of $x$ and $z$ coordinates of the global frame $W$ by $\hat{e}_x$ and 
$\hat{e}_z$, respectively. We let the position of the center of mass 
and the velocity of the microswimmer in 
the inertial frame $W$ be given by $p=[p_\text{x},\,p_\text{z}]^{\top}$ and 
$v=[v_\text{x},\,v_\text{z}]^{\top}$, respectively. We denote the angle of 
the center of mass (COM) position vector in the inertial coordinate frame by $\theta$. Therefore, 
\begin{equation}\label{eq:theta}
\theta := \text{atan2}(p_\text{z},p_\text{x}). 
\end{equation}
%
\begin{remark}
In this paper, we are only interested in controlling the position of the 
microrobot and not its orientation in the $x-z$ plane. Indeed, our model has \emph{only} 
two degrees of freedom, namely, the COM Cartesian coordinates given by  
$p_\text{x}$ and $p_\text{z}$. The angle $\theta$ in~\eqref{eq:theta} 
and the magnitude $\|p\|$ are the polar coordinates of the 
position vector $p=[p_\text{x},\,p_\text{z}]^{\top}$. \hfill$\triangle$
\end{remark}
%
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.425]{./figures/micro1.png}
	\caption{The configuration of a magnetic helical microrobot.}
	\label{fig:micro}
\end{figure}
%
%\vspace{-2ex}
The microrobot propulsion mechanism, which is based on transducing 
the external magnetic field energy to microrobot forward motion, can be described 
as follows. An external rotating uniform magnetic field, denoted by $H$ in 
Figure~\ref{fig:micro}, causes the magnetic helical microrobot 
to rotate about its axis. The resulting rotation about the helix axis in 
the ambient fluidic environment will then induce a screw-like motion and 
drive the microswimmer forward. Early analyses of helical propulsion of 
micro-organisms in fluids were carried out by~\cite{chwang1971note} 
and~\cite{purcell1977life}. In this paper, we use the 
control-oriented model developed in~\cite{mahoney2011velocity}. 


Using resistive force theory (RFT), Mahoney \emph{et al.}~\cite{mahoney2011velocity}  have 
derived the dynamical model of 3D helical microswimmers 
operating in low-Reynolds-number regimes. In 
this modeling approach, the velocity of each infinitesimally small segment of the 
helix is mapped to parallel and perpendicular differential fluid drag forces 
acting on the segment. Integrating the differential forces along the length of the helix in 
three dimensions, the fluidic force and  
torque acting on the helical part of the robot are obtained. 
Adding the fluidic forces acting on the head, the 
dynamical equations of motion of the microswimmer are obtained.

In this article we only consider the planar motion of the  
microrobot where the swimmer is rotated
around its helical axis and the direction of motion is 
perpendicular to the plane of microrobot rotation~\cite{zhang2009artificial}. 
Assuming that the microswimmer motion is confined to the $x-z$ plane, the dynamics of the 
planar microswimmer are given by (see~\cite{mahoney2011velocity} 
for detailed derivations)
%
\begin{eqnarray}\label{eq:2D_dyn}
\dot{p} & =&  A_{\theta}d_{\text{g}} + B_{\theta}u,
\end{eqnarray}
%
where 
\[
A_\theta = R_\theta A_h^{-1} R_{\theta}^{\top},\; 
B_\theta = -R_\theta A_h^{-1}B_h,\; d_{\text{g}}=-mg \ez.
\]

In the above, $R_{\theta}$ is the rotation matrix 
from the robot body-fixed frame $x_\tx{h}-z_\tx{h}$ to the inertial 
frame $W$. Furthermore, the constant matrices
\begin{equation}
\label{eq:ABstruct}
A_h = \begin{bmatrix} a_1 & 0 \\ 0 & a_2 \end{bmatrix},\; B_h = \begin{bmatrix} b_1 \\ b_2 \end{bmatrix}, 
\end{equation}
depend on the geometry of the helical microswimmer 
and the helix drag coefficients in its fluid environment. Moreover, $d_{\text{g}}$ is the 
net weight force (gravity minus buoyancy) that is acting on the 
robot in the inertial coordinate frame. Finally, $u$ is the frequency of 
rotation of the microrobot about the helix axis, which is proportional to 
the frequency of rotation of the external actuating uniform magnetic 
field (see Figures~\ref{fig:micro} and~\ref{fig:los}). 

%\begin{remark}
As it is shown in~\cite{mahoney2011velocity}, the constant 
control input vector $B_h$ in~\eqref{eq:2D_dyn} can be written as
\begin{equation}\label{eq:Bh}
B_h = ( \xi_{\parallel} - \xi_{\perp} ) B_h^{\prime}, 
\end{equation} 
where $\xi_{\parallel}$ and $\xi_{\perp}$ are the helix tangential 
and normal drag coefficients, and $B_h^{\prime}=[b_1^{\prime}, b_2^{\prime}]^\top\in\mathbb{R}^{2\times 1}$ is 
a constant vector with $b_1^{\prime}\neq 0$ and $b_2^{\prime}\neq 0$. The difference between the tangential and 
normal drag coefficients, i.e., $\xi_{\parallel}$ and $\xi_{\perp}$, plays a key role in control analysis, as 
discussed in Section~\ref{subsec:zerodyn}. 
%\end{remark}


The microrobot dynamics in~\eqref{eq:2D_dyn} can be written in 
the nonlinear affine control form 
%
\begin{eqnarray}\label{eq:2D_dynb}
\dot{p} & =&  f(p)+g(p)u,
\end{eqnarray}
%
\noindent where $p \subset \mathbb{R}^2$ is the state of 
the system and 
%
\[
f(p):= A_{\theta}d_\tx{g},\;\; 
g(p):= B_{\theta},\;\; \theta := \text{atan2}(p_z,p_x). 
\] 

==> section/intro.tex <==
\section{Introduction}
%
% reword and cite behkam
%
Swimming microrobots have attracted much attention in recent 
years due to their potential impact on 
medicine and micro-manipulation. In \emph{in vivo} medical 
applications, these robots 
can be used for performing safety critical therapeutic and 
diagnostic medical operations,  such as targeted drug delivery in hard-to-reach 
environments of the human body. In \emph{in vitro} or lab-on-a-chip 
applications, these robots can be used for 
cell manipulation and characterization as well as 
micro-fluid control. See, e.g.,~\cite{hong2017real,
	huang2016magnetic,nelson2010microrobots,
	abbott2009should,behkam2006design,behkam2007bacterial} 
for recent developments in this field. 

Microrobots can be categorized based on their morphologies and actuation 
methods.  Microrobot \emph{morphologies} such 
as cilia-like, eukaryotic-like, and helical morphologies are inspired 
from biological micro-organisms. The \emph{helical morphology}, 
which is inspired by bacterial flagella, is argued to provide 
the best overall choice for \emph{in vivo} 
applications~\cite{nelson2010microrobots,abbott2009should}. 

In addition to morphology, the type of actuator 
is another significant factor in microrobot design. To date, two classes of actuation methods 
have been proposed for swimming microrobot  propulsion 
in fluidic environments; namely, \emph{untethered magnetic actuation} 
in~\cite{abbott2009should,honda1996micro,nelson2010microrobots}, 
and \emph{molecular motors} in~\cite{behkam2006design,behkam2007bacterial, 
	kosa2007propulsion,kosa2008flagellar}. Actuators that 
use molecular motors pose numerous technological challenges in microfabrication as well as wireless power 
transmission and control. The untethered magnetic field actuation mechanisms, on the other hand, remove 
the need for replicating biological molecular motors and scale well in terms of 
microfabrication as well as wireless power and control.



Despite recent advances in microfabrication and actuation 
technologies for swimming magnetic microrobots, systematic design of automatic 
motion control algorithms for these microswimmers is an 
open problem to date. One of the major control limitations for magnetic 
helical microrobots is due to the existence of an upper limit on the rotational frequency of 
the robot body around its helical axis. The threshold frequency of helical microrobots' rotation, which 
keeps the robot in synchrony with the external rotating magnetic field, is known as the 
\emph{step-out frequency} beyond which the microrobot's 
velocity rapidly declines~\cite{nelson2010microrobots,abbott2009should}.  


%Being  susceptible to gravity and bodily 
%fluid flows, operating in low-Reynolds-number 
%regimes, low accuracy of measurement devices in 
%small scales, and actuator saturation are among a few interesting 
%challenges that arise in closed-loop control of this class of microrobots.
%Indeed, a magnetic helical microrobot needs to 
%maintain synchrony with external 
%rotating magnetic fields.  

% The mechanism underlying the helical magnetic microswimmers 
% can be described as follows. An external This helical rotation is induced by a rotating magnetic field 
% about the helix axis. The microrobot body rotation frequency, which is required for 
% maintaining synchrony with the rotating external magnetic field, cannot go over a certain  threshold.



The typical control approach in microrobot motion control 
literature relies on asymptotic tracking of suitably 
designed reference signals~\cite{vartholomeos2006analysis,
	arcese2013adaptive,zhang2017adaptive}. However, 
trajectory tracking controllers are subject to performance limitations, as demonstrated 
by~\cite{aguiar2005path}. An alternative approach 
is based on path following control schemes, which 
rely on making the desired paths invariant and attractive for the microrobot 
closed-loop dynamics. Few researchers have proposed path following controllers for 
magnetic microrobots~\cite{xu2015planar,khalil2017rubbing,oulmas2016closed}. However, the proposed 
path following schemes do not directly address the control input saturation 
issue. 


 
 
In this paper, we propose a path following control scheme that makes 
a given helical magnetic microrobot to converge to a desired straight 
line without violating the 
input saturation limits. Our feedback control solution is based on the
optimal decision strategy (ODS), which is a pointwise optimal control law 
that minimizes the deviation between the open-loop dynamics  vector field 
and a reference model vector field. Optimal decision strategies 
have been used in several applications such as controlling transients in power 
systems~\cite{thomas1976model}, and robotic manipulators with bounded 
inputs~\cite{spong1986control,spong1984control}. ODS-based 
strategies belong to the larger family of optimization-based 
nonlinear controllers~\cite{galloway2015torque,morris2015continuity,powell2015model,
	Ames17a,bouyar2017}, whose applications in robotics and driverless 
cars are growing, thanks in part to recent advancements in mobile computation 
power.  

Our proposed ODS-based control law for magnetic helical 
microrobots, which is cast as a quadratic program,  minimizes the difference 
between the microrobot velocity and a line-of-sight (LOS)-based reference vector 
field subject to input saturation constraints at each point of
the state space. The proposed reference vector 
field is inspired from the line-of-sight (LOS) path following laws that are 
widely used for underactuated marine craft control (see, e.g.,~\cite{fossen2003line,
	pettersen2001way,fossen2017direct}). 

\noindent\textbf{Contributions of the paper.} This paper contributes to solving 
the path following control problem for swimming microbots in 
\emph{two important ways}. First, the paper develops an LOS-based guidance 
law for swimming microrobots, inspired from the automatic ship steering 
literature~\cite{fossen2003line,pettersen2001way,fossen2017direct}. Second, 
using the LOS-based guidance law, this paper casts the control input 
computation as a quadratic program induced by the ODS 
framework~\cite{spong1986control}, which belongs to the wider class of real-time 
optimization-based controllers.  

The rest of this paper is organized as follows. First, we present the dynamical model of 
planar swimming helical microrobots in Section~\ref{sec:dynmodel}. Next, we formulate the 
straight-line path following control problem for a single swimming microrobot subject to control 
input constraints and outline our solution strategy in Section~\ref{sec:ContProb}. Thereafter, we present 
our ODS-based control scheme for swimming helical microrobots in Section~\ref{sec:Sol}. After 
presenting the simulation results in Section~\ref{sec:sims}, we 
conclude the paper with final remarks and 
future research directions in Section~\ref{sec:conc}.   
%

==> section/simStudies.tex <==
\section{Simulation Results}
\label{sec:sims}
%
In this section we present numerical simulation results to validate 
the performance of the ODS-based control method described in 
Section~\ref{sec:Sol}. We consider a helical magnetic microrobot  
with number of turns $n_{_\tx{h}}=4$, net effective mass  $m_{_\tx{h}}=8.9 \,\mu\tx{g}$, 
helix radius $r_{_\tx{h}}=0.5 \,\tx{mm}$, helix pitch angle $\theta_\tx{h}=45^{\circ}$, and 
magnetic head diameter $d_{_\tx{m}}=1 \tx{mm}$. Further, we assume that the microrobot is 
swimming in a fluid environment with viscosity 
$\eta_{\tx{v}}=0.98\, \tx{cP}$ and density $\rho = 970\, \tx{kg}/\tx{m}^3$ 
(close to that of water). The chosen parameters, which are 
taken from~\cite{abbott2009should} and~\cite{mahoney2011velocity}, satisfy the 
low-Reynolds-number regime condition and thus the dynamical model in~\eqref{eq:2D_dyn} 
is valid.   

Using the above microrobot and fluid parameters, the tangential and normal 
drag coefficients are found to be 
(see, e.g.,~\cite{mahoney2011velocity} for physical identities 
giving the relationship between the drag coefficients and the properties of 
the microswimmer and its ambient fluid environment)
%
\[
\xi_{\parallel} = 1.21 ,\; \xi_{\perp} = 2.03. 
\]
%
We would like the microrobot to follow the straight line 
\[
\mathcal{P}:=\{ p \in \mathbb{R}^2 : p = \tau\hat{e}_{_{\pi/4}} ,\, \tau\in \mathbb{R} \}, 
\]
subject to control input 
saturation limit $f_{_\tx{SO}}=24\,\tx{Hz}$. Since $\xi_{\parallel}\neq \xi_{\perp}$, from Proposition~\ref{prop:rel_deg}, 
we conclude that straight line $\mathcal{P}$ can be made invariant 
via feedback. The microrobot speed of line traversal, once constrained 
to $\mathcal{P}$, is $v^{\star} = 727\; \mu\tx{m}/\tx{sec}$, which has been 
computed using~\eqref{eq:microvel}. 

The look-ahead distance parameter $\Delta_\tx{LOS}$ in the LOS guidance law 
in~\eqref{eq:los} should be set equal to $v^{\star}/\alpha_{\tx{d}}$, where 
we have chosen $\alpha_{\tx{d}}=1$, if the 
accurate parameters of the robot and its environment are known. 
However, these parameters might not be known \emph{a priori}. In 
order to investigate the robustness of our proposed ODS-based scheme to 
parametric uncertainties, we design our control laws with 
approximate drag coefficients
%
\[
\hat{\xi}_{\parallel} = 1.10 ,\; \hat{\xi}_{\perp} = 1.31. 
\]
%
We use the ODS-based quadratic program in~\eqref{eq:ODS} with 
the positive definite matrix
\[
Q = \begin{bmatrix} 1 & 0 \\ -1 & 5 \end{bmatrix}. 
\]
%
In our simulation studies, we have initialized the microrobot 
position at $p(0)=[1\,\tx{mm},\; 1\,\tx{mm}]^{\top}$. In addition to 
the ODS-based scheme, we have also employed an input-output feedback linearizing 
control law, where the control input has been designed with 
no explicit consideration of saturation limits. However, during the 
simulations, we saturate this control input at $\pm f_{\text{SO}}$ whenever 
the values of the input-output feedback linearizing-based control law 
go beyond the saturation limits.     

Plots (a) and (b) in Figure~\ref{fig:path_nominal} depict the path of 
the microrobot and the control input time profile under the ODS-based 
scheme with $f_{\text{SO}}=24$ Hz. Plots (c) and (d) in 
Figure~\ref{fig:path_nominal} demonstrate the simulation 
results for the conventional input-output feedback linearizing control 
law that has been saturated with $f_{\text{SO}}=24$ Hz. As it can be 
seen from these plots, the swimming microrobt achieves a good path 
path-following performance under the ODS-based scheme in comparison with the 
saturated input-output feedback linearizing scheme where the microswimmer 
deviates more from the nominal path.  

In order to investigate the performance of our ODS-based scheme under 
smaller values of saturation limit, we have run simulations for 
step-out frequencies $f_{\text{SO}}=12$ Hz and $f_{\text{SO}}=6$ Hz, 
respectively. Figure~\ref{fig:path_nominal2} depicts the path of the 
microswimmer and the control input time profiles under these two 
frequencies. As it can be seen from the figure, a good path following 
can still be achieved once the saturation limit is halved from $24$ Hz 
to $12$ Hz. However, the ODS-based scheme fails once the saturation 
limit is halved from $12$ Hz to $6$ Hz. 

 

\begin{remark}[Sensing and Actuation]
In order to obtain the planar Cartesian coordinates of a given 
microrobot, off-the-shelf components such as 
microscopes and cameras combined with image-processing techniques
can be employed for imaging and localizing the 
microrobot~\cite{nelson2010microrobots}.  Three-axes Helmholtz coils, as 
described in~\cite{bell2007flagella}, can be used in order to generate  
rotating magnetic fields in arbitrary directions. \hfill$\triangle$
\end{remark}

% When the look-ahead distance parameter 
%is chosen to be twice the nominal speed on $\mathcal{P}$, the 
%microrobot converges to a line parallel to $\mathcal{P}$ but with a 
%small offset from the desired path. 


\begin{figure*}
	\centering
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.9\textwidth]{./figures/ODS_nominal_path.png} 
		\caption{}
	\end{subfigure}
	\quad\quad
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.9\textwidth]{./figures/ODS_nominal_u.png} 
		\caption{}
	\end{subfigure}
		\begin{subfigure}{0.4\textwidth}
			\includegraphics[width=0.9\textwidth]{./figures/OUTYsat_nominal_path.png} 
			\caption{}
		\end{subfigure}
		\quad\quad
		\begin{subfigure}{0.4\textwidth}
			\includegraphics[width=0.9\textwidth]{./figures/OUTYsat_nominal_u.png} 
			\caption{}
		\end{subfigure}
			\caption{Microrobot position and control input 
				time profiles under: (a, b) the ODS-based scheme 
				and (c, d) the input-output feedback 
				linearizing control law with $f_\text{SO}=24$ [Hz].}
			\label{fig:path_nominal}
\end{figure*}


\begin{figure*}
	\centering
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.98\textwidth]{./figures/ODS_half_path.png} 
		\caption{}
	\end{subfigure}
	\quad\quad
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.98\textwidth]{./figures/ODS_half_u.png} 
		\caption{}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.98\textwidth]{./figures/ODS_fourth_path.png} 
		\caption{}
	\end{subfigure}
	\quad\quad
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=0.98\textwidth]{./figures/ODS_fourth_u.png} 
		\caption{}
	\end{subfigure}
	\caption{Microrobot position and control input 
		time profiles under the ODS-based 
		scheme with: (a, b) $f_\text{SO}=12$ [Hz] and (c, d) 
		$f_\text{SO}=6$ [Hz].}
	\label{fig:path_nominal2}
\end{figure*}
	
%	\begin{subfigure}{0.4\textwidth}
%		\includegraphics[width=0.98\textwidth]{./figures/fig2l.png} 
%		\caption{}
%	\end{subfigure}
%    \begin{subfigure}{0.4\textwidth}
%    	\includegraphics[width=0.98\textwidth]{./figures/fig2pd.png} 
%    	\caption{}
%    \end{subfigure}

%	\label{fig:path}
%\end{figure*}

==> section/zerodyn.tex <==



